A Survey on Multi-Turn Interaction Capabilities of Large Language Models

Multi-turn interaction in the dialogue system research refers to a system's ability to maintain context across multiple dialogue turns, enabling it to generate coherent and contextually relevant responses. Recent advancements in large language models (LLMs) have significantly expanded the scope of multi-turn interaction, moving beyond chatbots to enable more dynamic agentic interactions with users or environments. In this paper, we provide a focused review of the multi-turn capabilities of LLMs, which are critical for a wide range of downstream applications, including conversational search and recommendation, consultation services, and interactive tutoring. This survey explores four key aspects: (1) the core model capabilities that contribute to effective multi-turn interaction, (2) how multi-turn interaction is evaluated in current practice, (3) the general algorithms used to enhance multi-turn interaction, and (4) potential future directions for research in this field.

==> tax_tree_applications.tex <==
\tikzstyle{my-box}= [
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=blue!15, text=black, align=left,font=\small,
    inner xsep=2pt,
    inner ysep
=4pt,
]
\begin{figure*}[ht]

    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\small,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=8.0em,font=\small,}{},
            where level=2{text width=8.0em,font=\small,}{},
            where level=3{text width=8.0em,font=\scriptsize,}{},
    [Applications, ver
        [Social Sector
            [Zhongjing~\shortcite{yang-etal-2024-zhongjing}, leaf, text width=42em]
        ]
        [Emotional Support
            [Meena~\shortcite{adiwardana-etal-2020-humanlike}{,} 
            PLATO-2~\shortcite{bao-etal-2021-plato}{,}
            NaturalConv~\shortcite{wang-etal-2021-naturalconv}{,}
            ESC~\shortcite{liu-etal-2021-towards}{,} 
            MultiESC~\shortcite{cheng-etal-2022-improving}{,}
            MISC~\shortcite{tu-etal-2022-misc}{,}
            PanGu-Bot~\shortcite{mi-etal-2022-pangubot}{,} \\
            BlenderBot~\shortcite{shuster-etal-2022-blenderbot3}{,}
            LaMDA~\shortcite{thoppilan-etal-2022-lamda}{,} 
            EVA2.0~\shortcite{Gu-etal-2023-eva2}{,}
            KEMI~\shortcite{deng-etal-2023-knowledge}{,}
            PLACES~\shortcite{chen-etal-2023-places}{,}
            SODA~\shortcite{kim-etal-2023-soda}{,} 
            Re3Dial~\shortcite{wen-etal-2023-re3dial}{,}  \\
            Hudeček et al.~\shortcite{hudecek-dusek-2023-large}{,}
            CESAR~\shortcite{aksu-etal-2023-cesar}{,} 
            Chen et al.~\shortcite{chen-etal-2023-controllable}{,} 
            SoulChat~\shortcite{chen-etal-2023-soulchat}{,}
            ExTES~\shortcite{zheng-etal-2024-self}{,} 
            ESCoT~\shortcite{zhang-etal-2024-escot}, leaf, text width=42em]
        ]
        [Content Generation
            [Chang et al.~\shortcite{chang-etal-2021-changing}{,}
            Rosa et al.~\shortcite{rosa-etal-2022-gpt}{,}
            C3~\shortcite{kottur-etal-2022-tellstorytod}{,}
            TiGAN~\shortcite{zhou-etal-2022-tigan}{,}
            TaleBrush~\shortcite{chung-etal-2022-talebrush}{,}
            FRIDE~\shortcite{zhong-etal-2023-fiction}{,} 
            CoEdIT~\shortcite{raheja-etal-2023-coedit}{,} \\
            LLM-as-a-tutor~\shortcite{han-etal-2024-llm}{,}
            PCQPR~\shortcite{guo-etal-2024-pcqpr}{,} Xinyu~\shortcite{wu-etal-2024-xinyu}{,}
            Tin et al.~\shortcite{tin-etal-2024-interactive}{,}
            Chat2Data~\shortcite{zhao-etal-2024-chat2data}{,} InkSync~\shortcite{laban-etal-2024-beyond}{,} \\
            HARM~\shortcite{zhang-etal-2024-holistic}{,} TheaterGen~\shortcite{cheng-etal-2024-theatergen}{,} DialogGen~\shortcite{huang-etal-2024dialoggen}, leaf, text width=42em]
        ]
        [Conversational Search
            [MuSIc~\shortcite{meng-etal-2023-music}{,} ConvSim~\shortcite{owoicho-etal-2023-exploiting}{,} CIRCLE~\shortcite{erbacher-soulier-2023-circle}{,} \\
            LeClari~\shortcite{liu-etal-2023-leclari}{,}
            MulClari-LLM~\shortcite{zhao-dou-2024-clarifying}{,} 
            ProMISe~\shortcite{butala-etal-2024-promise}{,}
            USi~\shortcite{sekulic-etal-2024-usi}{,}
            LAPS~\shortcite{joko-etal-2024-laps}{,} ChatQA~\shortcite{liu2024chatqa}{,} IM-RAG~\shortcite{yang-etal-2024-imrag}, leaf, text width=42em]
        ]
        [Personalization \\ \& Recommendation
            [UniCRS~\shortcite{wang-etal-2022-unicrs}{,} RecInDial~\shortcite{wang-etal-2022-recindial}{,} UniMIND~\shortcite{deng-etal-2023-unimind}{,} Chat-Rec~\shortcite{gao-etal-2023-chatrec}{,} RecLLM~\shortcite{friedman-etal-2023-leveraging}{,}  Liu et al.~\shortcite{liu-etal-2023-conversational}{,} \\
            He et al.~\shortcite{he-etal-2023-llmaszeroshot}{,}
            InstructRec~\shortcite{zhang-etal-2023-instructrec}{,}
            LLM-REDIAL~\shortcite{liang-etal-2024-llm}{,}
            MACRS~\shortcite{fang-etal-2024-multiagentcrs}{,} MG-CRS~\shortcite{zhang-etal-2024-mgcrs}{,} ChatCRS~\shortcite{li-etal-2024-incorporating}, leaf, text width=42em]
        ]
    ]
\end{forest}
}
    \caption{Relevant works on Multi-Turn Interaction Organized by Core Capabilities and Downstream Applications}
    \label{fig:organize-work-by-task}
\end{figure*}
